Simulation Scenarios in One-Dimensional Self-Gravitating System

We study and compare different numerical differential equation solvers on the basis of numerical complexity, energy conservation, and stable solution in phase-space for the Simple Harmonic Oscillation (SHM) problem. We conclude and show that the Leapfrog method is the best for our problem. We solve Poisson's equation in gravity on the computation grid by the finite difference method and Fourier method. We solve Poisson's equation for source not in a grid point by cloud-in cell method. Finally, we simulate one-dimensional self-gravitating system and show the evolution of the system via phase-space trajectories.

==> FrontMatter/acknowledgements.tex <==
\thispagestyle{plain}

\begin{center}
 \Large {\bf \uppercase{Acknowledgements}}
\end{center}

\vspace{3\baselineskip}

\noindent
plenty of waffle, plenty of waffle, plenty of waffle, plenty of waffle, plenty of waffle, plenty of waffle, plenty of waffle, plenty of waffle.

\noindent
\vspace{\baselineskip} \\
\textbf{\myname} \\
IIT Kharagpur \\
Date:

==> FrontMatter/certificate.tex <==
\thispagestyle{plain}

\begin{multicols}{2}
 \flushleft
 \includegraphics[width=20mm]{Images/iitkgplogo.jpg}
 \columnbreak
 \par
 Department of \mydep \\
 Indian Institute of Technology, Kharagpur \\
 India - 721302
\end{multicols}

\vspace{0.5\baselineskip}
\hrule
\vspace{3\baselineskip}

\begin{center}
{\Large {\bf \uppercase{Certificate}}}
\end{center}

\vspace{\baselineskip}

\noindent This is to certify that we have examined the thesis entitled {\bf \mytitle}, submitted by {\bf \myname}(Roll Number: {\textit{\myrollno}}) a postgraduate student of {\bf Department of \mydep}  in partial fulfillment for the award of degree of \mydegree. We hereby accord our approval of it as a study carried out and presented in a manner required for its acceptance in partial fulfillment for the Post Graduate Degree for which it has been submitted. The thesis has fulfilled all the requirements as per the regulations of the Institute and has reached the standard needed for submission.
\vspace{3\baselineskip}
\begin{flushright}
\begin{minipage}[c]{0.45\textwidth}
\centering
\hrule 
\vspace{0.5\baselineskip}
{\Large \bf Supervisor} \\
\flushleft{\large \textbf{Department of \mydep} \\
Indian Institute of Technology, Kharagpur}
\end{minipage}
\end{flushright}
\vspace{\baselineskip}

\noindent
{\large \bf Place: Kharagpur} \\
{\large \bf Date: }

==> FrontMatter/dedication.tex <==
\thispagestyle{empty}

\pagebreak
\hspace{0pt}
\vfill
\centering
Dedicated to \\
my mother \\
\textbf{\dedicationNamea} \\
\vspace{0.2cm}
and \\
my father \\
\textbf{\dedicationNameb}
\vfill
\hspace{0pt}
\pagebreak
